EvalAI: Towards Better Evaluation Systems for AI Agents

We introduce EvalAI, an open source platform for evaluating and comparing machine learning (ML) and artificial intelligence algorithms (AI) at scale. EvalAI is built to provide a scalable solution to the research community to fulfill the critical need of evaluating machine learning models and agents acting in an environment against annotations or with a human-in-the-loop. This will help researchers, students, and data scientists to create, collaborate, and participate in AI challenges organized around the globe. By simplifying and standardizing the process of benchmarking these models, EvalAI seeks to lower the barrier to entry for participating in the global scientific effort to push the frontiers of machine learning and artificial intelligence, thereby increasing the rate of measurable progress in this domain.

==> definitions.tex <==
% consistent formatting for quoting in the paper
\newcommand{\myquote}[1]{\emph{`#1'}}
\newcommand{\myapprox}{{\raise.17ex\hbox{$\scriptstyle\sim$}}}
% consistent bold starts
\newcommand{\xhdr}[1]{\vspace{3pt}\noindent\textbf{#1}}

% Definitions for referring to figure, section, table, equation
% (used uniformly thoughout)
\newcommand{\reffig}[1]{Fig.~\ref{#1}}
\newcommand{\refsec}[1]{Sec.~\ref{#1}}
\newcommand{\reftab}[1]{Tab.~\ref{#1}}
%\newcommand{\refeq}[1]{Eq.~\ref{#1}}


==> sections/future_work.tex <==
\section{Future Work}
With the wide-spread applications of AI systems in the wild, we not only need to benchmark models in terms of its accuracy, but also in terms of  it's computational efficiency and memory overhead. We want to build a benchmark tool such that models can be evaluated on different hardware - mobile hardware, embedded systems and 

\subsection{Centralized leaderboard to measure state-of-the-art on all AI benchmarks}
\subsection{Social platform around EvalAI}


